Dispatching Odyssey: Exploring Performance in Computing Clusters under Real-world Workloads

Recent workload measurements in Google data centers provide an opportunity to challenge existing models and, more broadly, to enhance the understanding of dispatching policies in computing clusters. Through extensive data-driven simulations, we aim to highlight the key features of workload traffic traces that influence response time performance under simple yet representative dispatching policies. For a given computational power budget, we vary the cluster size, i.e., the number of available servers. A job-level analysis reveals that Join Idle Queue (JIQ) and Least Work Left (LWL) exhibit an optimal working point for a fixed utilization coefficient as the number of servers is varied, whereas Round Robin (RR) demonstrates monotonously worsening performance. Additionally, we explore the accuracy of simple G/G queue approximations. When decomposing jobs into tasks, interesting results emerge; notably, the simpler, non-size-based policy JIQ appears to outperform the more "powerful" size-based LWL policy. Complementing these findings, we present preliminary results on a two-stage scheduling approach that partitions tasks based on service thresholds, illustrating that modest architectural modifications can further enhance performance under realistic workload conditions. We provide insights into these results and suggest promising directions for fully explaining the observed phenomena.

==> reviews.tex <==
Review #6A

Points to improve
scalability seems week, how to scale ?

Comments for authors
The paper reports that the performance of the two-stage system declines with larger server counts due to first-stage bottlenecks. Authors should mention how this could involve scaling the number of servers in the first stage based on real-time workload demands.


Review #6B

Points to improve
The paper's results are in line with the common understanding of the issues in real-world cluster scheduling, which detracts from the novelty of the findings. The main contribution, a two-stage dispatcher policy, requires task preemption and migration, functionalities whose implications are not discussed elsewhere in the paper and which might somehow bias the simulated comparison.


Review #6C

Points to improve
The presentation is somewhat confusing in regards to the main contributions of the paper. In the abstract, the focus is on the simulation-based trace analysis, which is in line with the bulk of the paper. The introduction also presents the 2-stage scheduling policy, which is discussed in detail at the end of the paper. I suggest the authors revise this to make the abstract, introduction and body more in agreement in the message regarding the 2-stage policy.
Comments for authors
The paper is well written and generally easy to follow.

In Section III, it is not completely clear how the expressions are obtained. While [20] is mentioned as the basis for these results, it should be stated whether these results are readily available in [20] or elsewhere. I assume this to be the case, as otherwise more details are needed for the derivation, but the paper passes this point rather quickly.

I think there are several interesting insights in the paper that could also be highlighted. For instance, the fact that the authors try several configurations with the shuffling of IATs and service times, until they find a setup where the models' predictions and the simulations match, revealing that the correlation in service times plays a critical role. This could be better highlighted in the introduction.

In the paper the standardized load is always 0.8, and this selection is not discussed. Do the results in the paper change if this load changes? Is this value selected for any particular reason?

In the discussion of Figure 10, a comparison is made of a 10-server cluster with a 1000-server cluster. I am not sure is this comparison is appropriate or at least it is not clear from the text how to interpret it.

Also regarding Figure 10, no information is provided as to the values of n_1, n_2 and theta. Are these somewhat fixed for any value of n? Or are they independently selected for each value of n?


Review #6D


Points to improve
Regarding results shown in Figure 10, which are the values set for theta and n_1? Furthermore, regarding the same results from Fig. 10, it would be interesting to see how the performance is affected under different values of theta (keeping the same value of n_1) and different values of n_1 (keeping the same theta). Finally, how would the expected performance be when JIQ and LWL are used in a two stage architecture?

